Dropout as data augmentation

Dropout is typically interpreted as bagging a large number of models sharing parameters. We show that using dropout in a network can also be interpreted as a kind of data augmentation in the input space without domain knowledge. We present an approach to projecting the dropout noise within a network back into the input space, thereby generating augmented versions of the training data, and we show that training a deterministic network on the augmented samples yields similar results. Finally, we propose a new dropout noise scheme based on our observations and show that it improves dropout results without adding significant computational cost.

==> text/discussion.tex <==
The plots showing the sparsity of hidden layer representations against the noise levels are shown in Figure \ref{fig:noise_sparsity}. In that figure only plots
corresponding to the random noise scheme experiments are shown where it can be observed that the sparsity of a given hidden layer representation is proportional 
to the level of noise applied to its input. The same observation of proportionality was made also in the case of dropout experiments.

To show that the proportionality between noise level and sparsity is not limited to using dropout noise, we performed an additional experiment using Gaussian noise
for corruption. We trained a two-layered MLP with $2500-1250$ hidden units on MNIST dataset using zero-mean additive Gaussian noise for input corruption.
The standard deviation of the Gaussian is varied to be in $[0.,0.2,.0.4,0.6]$ and corresponding layer-1 sparsity is shown in figure \ref{fig:noise_sparsity}.

Results from table \ref{tab:pnoise} suggest that Dropout can be replicated
by projecting the noise back into the input and training deterministically
a neural network on this generated data. There is not significant drop in 
accuracy, it is even slightly better than Dropout in the case of CIFAR10.
This support the idea that dropout can be seen as data augmentation. 
Furthermore, it suggests that local dynamics that could avoid co-adaptation
of neurons do not have a significant effect in the training of a neural network.

In figure \ref{fig:compare_response} we plotted the intermdiate layer representation of a 1000-2000-3000 hidden unit network trained with dropout corruption on CIFAR-10. 
We computed the intermediate layer representation of four different inputs \footnote{All the inputs are classified correctly.}
, i.e., a training sample $x_1$, corrupted version of it termed $\tilde{x}_1$, $x_2$;
another sample from the same class as that of $x_1$ and a sample from different class $x_3$. It can be observed from the figure that the 
representations of corrupted input $\tilde{x}_1$ and the one from the same class $x_2$ differ in a similar way from the representation of $x_1$
while being a lot different from that of $x_3$. This suggests that certain level corruption in hidden layers is similar to sampling a new input from the same class.






% Plots from figure \ref{fig:bias} shows first layer biases learned with 
% different activation functions. It can be observed that for all the networks, 
% the magnitude of negative bias increases with input noise level. Additionally,
% figure \ref{fig:spar_exps} shows that mean population sparsity of the 
% first layer activations is also proportional to input noise level.
% Those observations can be generalized to any layer of the network, where 
% previous layers activations are considered as the input. We observed that for 
% any given layer of the network, the sparsity and negative biases are 
% proportional to the noise level of their corresponding input.

% In section \ref{sec:dataaug}, we argued that increasing number of training 
% samples results in sparser representations and our experiments support this
% as seen in figure \ref{fig:spar_data_aug} c). Furthermore, figures 
% \ref{fig:noise_sparsity} a) and b) show that dropout noise applied on the
% input produces a similar sparsification effect than increasing number of
% training data.

% This further supports our hypothesis on the relationship between data samples 
% and sparsity. However, one can notice a discrepancy between figures 
% \ref{fig:spar_exps} and \ref{fig:spar_data_aug} where mean population sparsity
% evolves much faster in the former one. It is important to note that noise is 
% applied on-line in experiments of figure \ref{fig:spar_exps} while 
% pre-generated off-line in the latter. Because of this, models from former
% experiments have seen many more different noisy examples. This, we 
% believe, partly explains the discrepancy.

The classification results presented in figures \ref{fig:dropout_noise},
show that random noise levels gives better performance overall. 
As explained in section \ref{subsec:randomnoise}, random noise levels introduce
richness in noise distribution which in turn transform training data 
with more diversity. It should be trivial then, that random noise, by 
producing more diverse data transformations is improving training and
our results support this.

% such that it better covers 
%augmentation transformation yields better training, results with richer 
%random noise schemes supports the hypothesis that multiplicative noise has a 
%similar effect as augmenting data. 
%\fbox{Is it me or the inference here is weak somehow?}
%When considered as a data augmentation 
%transformation, this   which better covers 
%Again, This shows that random noise levels which implies more augmented data samples
%results in a more generalized model and therefore better performance.

% An interesting fact that emerged from our experiments can be observed in 
% tables \ref{tab:dropout}, \ref{tab:dropoutTanhRec}, \ref{tab:cifarrandomReLU} 
% and \ref{tab:cifarrandomRTanh}. In every experiments, models with ReLU 
% activation functions are on-par with models using rectified-tanh. As the latter
% function quickly saturates to 1, it seems that the linear part of the ReLU
% is not fully exploited. Moreover, this is consistent with the hypothesis
% that a sparse representation is tiling input sub-regions, i.e, each activation
% represents whether an example is within a given sub-region or not. Nonetheless, 
% more experiments should be conducted to support those speculations. Namely, 
% the importance of the linear part of rectified-tanh should be studied 
% in order to safely infer that optimal activations are essentially close to 
% binary.
% 
%it can observed that the performance when
%using Rectified-Tanh non-linearity is on par with Relu based networks. This shows that in discriminative settings involving
%highly non-linear or discontinuous data manifolds a binary encoding is sufficient as input space tiling is the best possible solution.

% Finally, PGN which appears to be an approximation of DropConnect yields
% slightly better results than Dropout in most of our
% experiments (see tables \ref{tab:dropout}, \ref{tab:gaussian}, 
% \ref{tab:rndnoise} and \ref{tab:non_linear}).


==> text/experiments_new.tex <==
\subsection{Training deterministically with noise projected back into input}
We ran a series of experiments with Multi-Layer-Perceptron (MLP) architectures on the MNIST and CIFAR-10 datasets to study the effect of replacing dropout by back-projected inputs.
Each MLP consists of two hidden layers with ReLU units followed by a {\it softmax} layer. We experimented with four different MLP architectures each one with a different number of units in the hidden layers: 
2500-2500, 2500-1250, 1500-1500 and 1500-750. The MNIST dataset consists of $60000$ training samples and $10000$ test samples. We split the training set into a set of $50000$ samples for training 
and $10000$ for validation. Each network is trained for $501$ epochs and the best model based on validation error is selected. Later the best model is further trained on the complete training set 
of $60000$ samples (training + validation split) for another $150$ epochs. The mean error 
percentage for the last $75$ epochs is used for comparison. 

We also ran experiments on the CIFAR-10 permutation invariant task using the same MLPs described above. The dataset consists of 
$50000$ training samples and $10000$ test samples. We use PCA based dimensionality reduction without whitening as preprocessing scheme. 
We used the same approach as that in the MNIST experiments to train the networks and for reporting the performances.

To test our hypothesis on non-visaul data we experimented on a version of TIMIT dataset. TIMIT is a 
phonetically transcribed corpus of speech spoken by North American speakers. We used dataset from 
\cite{cotter2011gpu}. They used MFCC features extracted from every 10ms frame of a subset of the TIMIT dataset, 
together with the first two derivatives of the features, for the task of classification of the stop consonants for every frame.
The dataset consists of 63881 train samples and 22257 test samples.

We used a fixed hidden noise level of $0.5$ and the input noise level varying from $0.2$ to $0.6$ with increments of $0.2$ (for each experiment)
in our reference models and the same values to compute back-projected inputs.
At each epoch, an $x^*$ is generated for each training sample. It proved to be possible to find 
good $x^*$ approximations for the entire
network at once for a 2-hidden layer network. Thus, we trained on $x$ and $x^*$ solely rather than $x$, $x^{(1)^*}$ and $x^{(2)^*}$ as it gave a significant speed up. 
For simplicity, the network is trained on $x$ for an epoch than on $x^*$ for an epoch. All $x^*$ 
are generated with parameter values of the model at the beginning of the epoch.

Noisy inputs $x^*$ are found using stochastic gradient descent. 20 learning 
steps are done with a learning rate of 300.0 for first hidden layer
and 30 for second hidden layer. The results for these experiments are shown in figure \ref{fig:pnoise}.
The images generated via back projection of noise in the network are shown in figure \ref{fig:pnoise_ims}.

% \begin{table*}[t]
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcc}
%  Experimental setup    & MNIST  & CIFAR-10 \\ \hline
%  Dropout on input      & 1.12\% & 40.9\% \\
%  Dropout on input+hidden & 0.95\% & 39.0\%\\
%  Noise projection      & 0.99\% & 37.9\%\\
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \caption{Test accuracy on permutation invariant MNIST and CIFAR-10 (2500-1250 hidden units with 0.2 dropout input noise and 0.5 hidden layer dropout noise where applicable). Noise on CIFAR-10 is applied to the PCA representation.}
% \label{tab:pnoise}
% \end{table*}

\begin{figure}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/cifar_Dropout__error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/mnist_Dropout__error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/timit_Dropout__error_plot.png}} \\
 
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/cifar_DataAug1__error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/mnist_DataAug1__error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/timit_DataAug1__error_plot.png}}
 \caption{Error percentages on the MNIST and CIFAR-10 datasets using MLP architectures trained with different corruption schemes.
 {\bf Row-1}: Experiments using dropout. {\bf Row-2}: Experiments using noise back projection. {\bf Column-1}: CIFAR-10
 {\bf Column-2}: MNIST. {\bf Column-3}: TIMIT. Noise on CIFAR-10 is applied to the PCA representation.}
 \label{fig:pnoise}
\end{figure}



\begin{figure}
 \subfigure[Epoch 1 ]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_cifarRelu_1500_epoch0.png}}
 \subfigure[Epoch 10]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_cifarRelu_1500_epoch10.png}}
 \subfigure[Epoch 20]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_cifarRelu_1500_epoch20.png}}
 \subfigure[Epoch 30]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_cifarRelu_1500_epoch30.png}} \\
 
 \subfigure[Epoch 1 ]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_mnistRelu_1500_epoch0.png}}
 \subfigure[Epoch 10]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_mnistRelu_1500_epoch10.png}}
 \subfigure[Epoch 20]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_mnistRelu_1500_epoch20.png}}
 \subfigure[Epoch 30]{\includegraphics[width=0.24\textwidth]{figures/DataAug1_mnistRelu_1500_epoch30.png}} \\
 \caption{Images generated using back projection of noise in a $1500-750$ network using 0.2 input and 0.5 hidden noise levels trained on.
 {\bf Row-1}: CIFAR-10. {\bf Row-2}: MNIST datasets.}
 \label{fig:pnoise_ims}
\end{figure}


Results from the figure \ref{fig:pnoise} suggest that Dropout can be replicated
by projecting the noise back into the input and training 
a neural network deterministically on this generated data. There is not significant drop in 
accuracy, it is even slightly better than Dropout in the case of CIFAR-10.
This support the idea that dropout can be seen as data augmentation. 
Furthermore, it suggests that local dynamics that could avoid co-adaptation
of neurons may not play a significant role in the training of the networks.

% In figure \ref{fig:compare_response} we plotted the intermediate layer representation of a 1000-2000-3000 hidden unit network trained with dropout corruption on CIFAR-10. 
% We computed the intermediate layer representation of four different inputs \footnote{All the inputs are classified correctly.}
% , i.e., a training sample $x_1$, corrupted version of it termed $\tilde{x}_1$, $x_2$,
% another sample from the same class as that of $x_1$ and a sample from different class $x_3$. It can be observed from the figure that the 
% representations of corrupted input $\tilde{x}_1$ and the one from the same class $x_2$ differ in a similar way from the representation of $x_1$
% while being a lot different from that of $x_3$. This suggests that certain level corruption in hidden layers is similar to sampling a new input from the same class.


\subsection{Random-dropout experiments}
We ran a series of experiments with Multi-Layer-Perceptron (MLP) architectures on the MNIST and CIFAR-10 datasets to compare dropout.
Each MLP consists of two hidden layers with ReLU units followed by a {\it softmax} layer. We experimented with three different MLP architectures 
each one with a different number of units in the hidden layers: 2500-625, 2500-1250 and 2500-2500.
Each network is trained and validated in the as same way mentioned in previous section.

First, we evaluated the dropout noise scheme by training the MLPs with a fixed hidden noise level of $0.5$ and the input noise level varying from $0.0$ to $0.7$ with increments of $0.1$ for each experiment.
In the second experiment, we fixed the input noise level at $0.2$ and the hidden noise level is varied from $0.0$ to $0.7$, again with an increment of $0.1$. 
In the final set of experiments we use the Random Dropout noise scheme using the same noise level at input and hidden layers. 
The noise level in this case is a range $[0,x]$ where $x$ is varied from $0.0$ to $0.8$ with increment $0.1$. % resulting in multiple experiments.
The classification performances corresponding to the all the experiments on both the datasets are reported in Figure \ref{fig:dropout_noise}.

\begin{figure}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/cifar_var_inputnoise_error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/cifar_var_hiddennoise_error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/cifar_var_RndDrop_error_plot.png}} \\
 
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/mnist_var_inputnoise_error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/mnist_var_hiddennoise_error_plot.png}}
 \subfigure[]{\includegraphics[width=0.33\textwidth]{figures/mnist_var_RndDrop_error_plot.png}}
 \caption{Error percentages on the MNIST and CIFAR-10 datasets using MLP architectures trained with different corruption schemes.
 {\bf Row-1}: Experiments on CIFAR-10. {\bf Row-2}: Experiments on MNIST. {\bf Column-1}: Using dropout with varying input noise and fixed hidden noise of 0.5. 
 {\bf Column-2}: Using dropout with varying hidden noise with fixed input noise of 0.2. {\bf Column-3}: Using Random-dropout with varying noise range $[0,x]$ used at hidden and input layers.}
 \label{fig:dropout_noise}
\end{figure}

% \begin{figure}
%  \includegraphics[width=1.\textwidth]{figures/Layer2_outputs_compare.png}
%  \caption{Comparing layer-2 responses of a 1000-2000-3000 unit network trained with dropout corruption on CIFAR-10. $x_1$: Original train sample without dropout. $\tilde{x}_1$: $x_1$ when using regular dropout in the network.
%  $x_2$: Different sample from same class as that of $x_1$. $x_3$: Sample from a different class. For $x_1$, the indices of hidden representation are sorted in increasing order of 
% the corresponding response and the same order is used for hidden representations in other cases.}
%  \label{fig:compare_response}
% \end{figure}




==> text/noise_old.tex <==
Common types of artificial noise considered in artifical neural networks are typically 
additive or multiplicative. Additive noise is independent of input intensity 
and synaptic connection strenghs while multiplicative is dependent on them.
For example, given an input vector $\vec{x}$, a weight vector $\vec{w}$ and a noise distribution $e$,
$\vec{w}^{\mathrm{T}}\vec{x} + e$ is termed additive if $e$ is independent of $\vec{x}$ and $\vec{w}$ and multiplicative
if $e \propto$ to the intensities of $\vec{x}$ and $\vec{w}$.

Dropout \cite{dropout} is a technique where a fraction of hidden units in a deep network are randomly turned off while training.
Given an input vector $\vec{x}$ to a layer and an $N$-dimensional weight vector $\vec{w}_n$. The hidden response 
corresponding to filter $\vec{w}_n$ before non-linearity can be written as

\begin{equation}
    \vec{h}_n = \sum_i x_i w_{n,i} + b = \vec{w}_n^\mathrm{T}\vec{x} + b_n
\end{equation}

Using dropout involves multiplying $\vec{x}$ with a binary mask sampled with probability $p$. Most often, the probability used is $0.5$ 
which implies half of the input dimensions (or hidden units if input is from previous layer) are dropped. To compensate the loss of
magnitude the active dimensions are scaled by $\frac{1}{p} = 2.$. The new hidden value can be written as,

\begin{equation}
  h_{n} = \vec{w}_n^\mathrm{T}(\vec{r} \odot \vec{x}) + b_n
\end{equation}

where $P(r_i = 1) = 0.5$. Similarly, the DropConnect can be formalized as

\begin{equation}
  h_{n} = (\vec{r}_n \odot \vec{w}_n)^\mathrm{T} \vec{x} + b_n
\end{equation}

Dropconnect can be thought of as having a different input binary mask corresponding to each weight vector where Dropout only has one.
Even though the multiplication of $\vec{r}$ with the input or hiddens suggests it is a multiplicative noise, it is not clear at first glance
how this noise is dependent on input intensity and synaptic connection strentghs. 
As shown by \cite{dropconnect}, this noise scheme, can be approximated via moment 
as a Gaussian noise distribution on the hidden units, which gives equation \ref{eq:gaussiandropconnect}.
\begin{equation} \label{eq:gaussiandropconnect}
    h_{n} =  \vec{w}_n^\mathrm{T}\vec{x} + (\vec{w}_n^2)^\mathrm{T}\vec{x}^2 \mathbf{\mathcal{N}}\left(0, p(p-1)\right) + b_n
\end{equation}

where $\vec{w}_n^2$ and $\vec{x}^2$ are element-wise squares.
From equation \ref{eq:gaussiandropconnect} it is clear that the noise variance will span with 
$(\vec{w}_n^2)^\mathrm{T}\vec{x}^2$. Interestingly, the variance
is proportional to intensity of reponse. We used equation \ref{eq:gaussiandropconnect} 
in our experiments rather than a binary mask, but replaced expression $p(p-1)$ with
hyperparameter $\sigma^2$. We term this approach as "Proportional Gaussian Noise" (PGN). The hidden response when
using PGN can be written as

\begin{equation} \label{eq:PGN}
 h_{n} =  \vec{w}_n^\mathrm{T}\vec{x} + (\vec{w}_n^2)^\mathrm{T}\vec{x}^2 \mathbf{\mathcal{N}}\left(0, \sigma^2\right) + b_n
\end{equation}

%\subsection{Update rules}
%
%Since symbolic differentiation tools such as Theano are used in machine 
%learning, computing the gradient by hand is avoided unless there is an 
%analytical use for it. However, the presence of a squared 
%weight in equation \ref{eq:MYNOISE}
%induces an interesting property into the derivative of the loss function 
%given the weights. Therefore, it is worth deriving the equation to analyse it.
%%$\displaystyle\frac{\partial \mathcal{L}_n}{\partial W^{(\l)}}$
%
%Let $\mathcal{L}$, an arbitrary loss function, $a^{(\l)}$, an arbitrary activation function for layer $\l$, $A_n^{(\l)}$ the activation of
%hidden layer $\l$ on the $n$-th exemple and $L$ the total number of layers including input and output layers
%\footnote{The input and output layers are typically $X$ and $softmax()$ 
%    respectively for multiclass classification tasks. Thus, $A^{(0)}=X$ and $A^{(L)} = softmax(H^{(L)})$. $H^{(0)}$ does not exist.}.
%
%We need $\displaystyle\frac{\partial \mathcal{L}_n}{\partial W^{(\l)}}$ in order to compute the update rule on $W^{(\l)}$. By the chain-rule theorem,
%
%\begin{equation} \label{eq:gradientMYNOISE}
%  \frac{\partial \mathcal{L}_n}{\partial W^{(\l)}} = 
%  \frac{\partial H_n^{(\l)}}{\partial W^{(\l)}}^T
%  \left[\frac{\partial \mathcal{L}_n}{\partial H_n^{(L)}}
%  \left(
%  \prod_{i=1}^{L-\l} \left[\frac{\partial H_n^{(L-i+1)}}{\partial A_n^{(L-i)}}\right]^T
%  \frac{\partial A_n^{(L-i)}}{\partial H_n^{(L-i)}}
%  \right)
%  \right]
%\end{equation}
%
%We then derive $\frac{\partial H_n^{(\l)}}{\partial W^{(\l)}}$ in particular to reveal something interesting,
%
%\begin{equation}
%    \frac{\partial H_n^{(\l)}}{\partial W^{(\l)}} = A_n^{(l-1)} + 2\left(A_n^{(l-1)}\right)^2W^{(l)}\mathbf{\mathcal{N}}(0, \sigma^2)
%\end{equation}
%
%Presence of $W^{(\l)}$ in $\frac{\partial H_n^{(\l)}}{\partial W^{(\l)}}$ 
%(and consequently in equation \ref{eq:gradientMYNOISE}) suggests that some kind 
%of penalty is applied on the weights during learning. More experiments should be done to 
%better understand the effect of this particular gradient on learning. 
%
%(** I'm not satisfied by this subsection... -\_- Xavier **)
%
%\begin{align}
%    \frac{\partial \mathcal{L}_n}{\partial W^{(\l)}} = & 
%  \left(A_n^{(l-1)}\right)^T
%  \left[\frac{\partial \mathcal{L}_n}{\partial H_n^{(L)}}
%  \left(
%  \prod_{i=1}^{L-\l} \left[\frac{\partial H_n^{(L-i+1)}}{\partial A_n^{(L-i)}}\right]^T
%  \frac{\partial A_n^{(L-i)}}{\partial H_n^{(L-i)}}
%  \right)
%  \right] \nonumber \\
%& + \left(2\left(A_n^{(l-1)}\right)^2W^{(l)}\mathbf{\mathcal{N}}(0, \sigma^2)\right)^T
%\left[\frac{\partial \mathcal{L}_n}{\partial H_n^{(L)}}
%  \left(
%  \prod_{i=1}^{L-\l} \left[\frac{\partial H_n^{(L-i+1)}}{\partial A_n^{(L-i)}}\right]^T
%  \frac{\partial A_n^{(L-i)}}{\partial H_n^{(L-i)}}
%  \right)
%  \right]
%\end{align}
%
%\begin{equation}
%  \frac{\partial \mathcal{L}_n}{\partial W^{(\l)}} =
%  \left(A_n^{(l-1)}\right)^T
%  \left[\frac{\partial \mathcal{L}_n}{\partial H_n^{(L)}}
%  \left(
%  \prod_{i=1}^{L-\l} \left[\frac{\partial H_n^{(L-i+1)}}{\partial A_n^{(L-i)}}\right]^T
%  \frac{\partial A_n^{(L-i)}}{\partial H_n^{(L-i)}}
%  \right)
%  \right]
%\end{equation}

% \fbox{\begin{minipage}{\textwidth}
%   Kishore's sketch
% \end{minipage}}
% 
% Dropout is a technique where certain fraction of hidden units in a deep network are randomly turned off while training.
% Given $X$ is an input vector to a layer and $W$ be one of the filters with $N$ dimensions. The hidden values before non-linearity corresponding
% to filter $W$ can be written as,
% \begin{equation}
%  h = \sum_i^N {s_i}
% \end{equation}
% where $s_i = x_iw_i$. Using dropout involves multiplying $X$ with a binary mask sampled with certain probability. Most often, the probability used is
% $0.5$ which implies half of the input dimensions are dropped. To compensate the loss the active dimensions are scaled by $2$. The new hidden value can
% be written as,
% 
% \begin{equation}
%  h_d = \sum_i^N {2s_ib_i}
% \end{equation}
%  where $P(b_i=1)=0.5$. Let us assume $A$ is set of indices where $b_i=1$ and $B$ a set where $b_i=0$ each with $N/2$ elements. $h_i$ can be written
%  as,
% \begin{equation}
%  h_d = \sum_{i\in A} {2s_i}
% \end{equation}
% 
% Based on the above notation of Dropout we present an alternative Guassian noise scheme which has a standard deviation dependent on input and weight strenghts.
% Assuming the hidden response without dropout $\sum_i^N {s_i}$ as mean we compute the standard deviation for the normal distribution of hidden responses with dropout.
% The total number of possible responses $T$ would be the number ways in which set $A$ can be drawn from total set of indices. The standard deviation can be computed as
% 
% \begin{eqnarray}
%  \sigma^2 & = & \frac{\sum_T(h - h_d)^2}{T} \\ \nonumber
%           & = & \frac{\sum_T(\sum_i^N {s_i} - \sum_{i\in A} {2s_i})^2}{T} \\ \nonumber
%           & = & \frac{\sum_T(\sum_{i\in B} {s_i} - \sum_{i\in A} {s_i})^2}{T} \\ \nonumber
%           & = & \frac{T \sum_{i} {(s_i)^2}}{T} \\ \nonumber
%           & = & \sum_{i} {(s_i)^2} 
% \end{eqnarray}
% 
% Hence an alternative way to get the similar effect as of dropout one could formulate the hidden response to be
% \begin{equation}
%  h_d=\mathcal{N}(\mu = \sum_i^N {s_i}, \sigma^2 = \sum_i^N {s_i^2})
% \label{Noisescheme}
% \end{equation}

In the next section we show how multiplicative noise acts as a strong regularization scheme by behaving as a data augmentation without domain knowledge.

